Evaluating Logical Generalization in Graph Neural Networks

Recent research has highlighted the role of relational inductive biases in building learning agents that can generalize and reason in a compositional manner. However, while relational learning algorithms such as graph neural networks (GNNs) show promise, we do not understand how effectively these approaches can adapt to new tasks. In this work, we study the task of logical generalization using GNNs by designing a benchmark suite grounded in first-order logic. Our benchmark suite, GraphLog, requires that learning algorithms perform rule induction in different synthetic logics, represented as knowledge graphs. GraphLog consists of relation prediction tasks on 57 distinct logical domains. We use GraphLog to evaluate GNNs in three different setups: single-task supervised learning, multi-task pretraining, and continual learning. Unlike previous benchmarks, our approach allows us to precisely control the logical relationship between the different tasks. We find that the ability for models to generalize and adapt is strongly determined by the diversity of the logical rules they encounter during training, and our results highlight new challenges for the design of GNN models. We publicly release the dataset and code used to generate and interact with the dataset at https://www.cs.mcgill.ca/~ksinha4/graphlog.

==> sections/notations.tex <==
\subsection{Items}

\begin{itemize}
    \item a World $W^k = \{\mathcal{R}, \{r_1,r_2,...,r_k\},G\}$ consists of $k$ different relations  $\{r_1,r_2,...,r_k\}$; a \textbf{knowledge base} $\mathcal{R}$, which is a set of unary and binary \textit{rules} using the relations
    \item a KB $\mathcal{R}$ contains a set of rules involving the relations in
    \begin{itemize}
        \item unary format : $r_i \rightarrow r_j$
        \item binary format (DataLog): $[r_i, r_j] \rightarrow r_k$
    \end{itemize}
    \item Given a world, we create $n$ unique graphs $G = (g_1, \ldots g_n)$ applying $\mathcal{R}$
    \item $\forall g_i \in G$,
    \begin{itemize}
        \item Entities $v_1 \ldots v_e$
        \item A path $p_{g_i}$ which is a walk from $v_{source} \rightarrow v_j \ldots \rightarrow v_{sink}$ which we term as the \textit{resolution path}. This is unique for each $g_i$.
        \item Target relation to predict $v_{source} \rightarrow v_{sink} = r_t(g_i)$
        \item Arbitrary noise paths
    \end{itemize}
    \item $f_R$ being the model we learn, which has $\theta_R$ parameters. This representation can be shared among all worlds, or we could learn a task specific $\theta_R$.
    \item $f_S$ is the \textit{signature function}, which has $\theta_S$ parameters. The idea is that the signature function provides a context vector for each world $W_i$ by having input $f_S(\hat{G}_{train})$. Here, $\hat{G}_{train}$ differs from $G_{train}$ by having the answers of the link prediction task within the graph. Ideally, this helps the model to learn the logical rules of the world. Also, $\hat{G}_{train}$ is a sampled subset of $G_{train}$.
    \item Unless otherwise specified, $f_R$ and $f_S$ are both implemented by a modified GAT \citep{velikovi2017graph} architecture to handle edge relations.
\end{itemize}

\subsection{Data Splits}

\begin{itemize}
    \item We create a train, validation and test split of worlds.
    \begin{equation}
        T_{train} = (W^k_1, \ldots W^k_a), \\ 
  T_{valid} = (W^k_{a+1}, \ldots W^k_b), \\ 
  T_{test} = (W^k_{b+1}, \ldots W^k_c)
    \end{equation}
    \item Within each world $W_i$, we have a train/valid/test split over the graphs : $G_{train}, G_{valid}, G_{test}$
    \item Sanity check $T_{train} = (W^k, \ldots, W^k), \\ T_{valid} = (W^k,\ldots, W^k), \\ T_{test} = (W^k,\ldots, W^k)$
\end{itemize} 

==> tables/maml_frozen.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|ll|ll|ll|ll|}
\hline
 &  & \multicolumn{2}{l|}{Frozen $f_r^*$} & \multicolumn{2}{l|}{Frozen $f_c^*$} \\ \cline{3-6} 
 &  & $k=10$ & $k=c_t$ & $k=10$ & $k=c_t$ \\ \cline{3-6} 
$f_r$ & $f_c$ & accuracy & accuracy & accuracy & accuracy \\ \hline
GAT & E-GAT & 0.134 & 0.366 & 0.093 & 0.234 \\
Param & E-GAT & 0.128 & 0.366 & 0.051 & 0.218 \\
GCN & E-GAT & 0.161 & 0.334 & 0.08 & 0.202 \\
GAT & RGCN & 0.081 & 0.383 & 0.073 & 0.317 \\
Param & RGCN & 0.084 & 0.307 & 0.072 & 0.264 \\
GCN & RGCN & 0.132 & 0.342 & 0.076 & 0.336 \\ \hline
\end{tabular}%
}
\caption{MAML ablation with pre-trained composition function $f_c^*$ and pre-trained Representation function $f_r^*$. Both are frozen and not allowed to update.}
\label{tab:my-table}
\end{table}

==> tables/multitask.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|ll|llll|ll|}
\hline
&  & $k=0$ & $k=5$ & $k=10$ & $k=c_t$ \\ \cline{3-6} 
$f_r$ & $f_c$ & accuracy & accuracy & accuracy & accuracy \\ \hline
GAT & E-GAT & 0.464 & 0.507 & 0.534 & 0.588 \\
Param & E-GAT & 0.459 & 0.497 & 0.512 & 0.572 \\
GCN & E-GAT & 0.401 & 0.456 & 0.503 & 0.545 \\
GAT & RGCN & 0.283 & 0.321 & 0.324 & 0.442 \\
Param & RGCN & 0.24 & 0.262 & 0.28 & 0.343 \\
GCN & RGCN & 0.307 & 0.327 & 0.378 & 0.429 \\ \hline
\end{tabular}%
}
\caption{Multitask setup - Inductive, zero shot, 5-shot, 10-shot and convergence}
\label{tab:my-table}
\end{table}

==> tables/multitask_frozen.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|ll|ll|ll|ll|}
\hline
 &  & \multicolumn{2}{l|}{Frozen $f_r^*$} & \multicolumn{2}{l|}{Frozen $f_c^*$} \\ \cline{3-6} 
 &  & $k=10$ & $k=c_t$ & $k=10$ & $k=c_t$ \\ \cline{3-6} 
$f_r$ & $f_c$ & accuracy & accuracy & accuracy & accuracy \\ \hline
GAT & E-GAT & 0.128 & 0.382 & 0.103 & 0.242 \\
Param & E-GAT & 0.098 & 0.356 & 0.422 & 0.485 \\
GCN & E-GAT & 0.068 & 0.333 & 0.067 & 0.31 \\
GAT & RGCN & 0.197 & 0.335 & 0.09 & 0.289 \\
Param & RGCN & 0.174 & 0.321 & 0.145 & 0.301 \\
GCN & RGCN & 0.155 & 0.29 & 0.123 & 0.329 \\ \hline
\end{tabular}%
}
\caption{Multitask ablation with pre-trained composition function $f_c^*$ and pre-trained Representation function $f_r^*$. Both are frozen and not allowed to update.}
\label{tab:my-table}
\end{table}

==> tables/supervised.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|ll|l|}
\hline
 &  & Inductive \\ \cline{3-3} 
$f_r$ & $f_c$ & accuracy \\ \hline
GAT & E-GAT & 0.655 \\
Param & E-GAT & 0.627 \\
GCN & E-GAT & 0.623 \\
GAT & RGCN & 0.548 \\
Param & RGCN & 0.457 \\
GCN & RGCN & 0.498 \\ \hline
\end{tabular}%
}
\caption{Supervised setup - Transductive and Inductive Reasoning}
\label{tab:supervised}
\end{table}
